An Introduction to Modern Enumerative Geometry with Applications to the Banana Manifold

The banana manifold $X_{\text{ban}}$ is a smooth projective Calabi-Yau threefold fibered over $\mathbb{P}^{1}$ by abelian surfaces. Each singular fiber contains a "banana configuration of curves" which generates the rank-three lattice $\Gamma$ of curve classes supported in the fibers of $X_{\text{ban}}\to\mathbb{P}^{1}$. The Donaldson-Thomas partition function of $X_{\text{ban}}$ in fiber classes was computed by J. Bryan (arXiv:1902.08695) to be the infinite product \[Z_{\text{DT}}(X_{\text{ban}})_{\Gamma}= \prod_{d_{1},d_{2},d_{3}\geq0}\prod_{k\in\mathbb{Z}}\big(1-Q_{1}^{d_{1}}Q_{2}^{d_{2}}Q_{3}^{d_{3}}t^{k}\big)^{-12c(||\underline{\bf{d}}||,k)}\] where $||\underline{\bf{d}}||=2d_{1}d_{2}+2d_{1}d_{3}+2d_{2}d_{3}-d_{1}^{2}-d_{2}^{2}-d_{3}^{2}$, and $c(||\underline{\bf{d}}||,k)$ are coefficients of the equivariant elliptic genus of $\mathbb{C}^{2}$. We observe that under a change of variables, $Z_{\text{DT}}(X_{\text{ban}})_{\Gamma}$ behaves formally like a Borcherds lift of the equivariant elliptic genus. The main result of this thesis is that the associated Gromov-Witten potentials $F_{g}$ in genus $g\geq2$ are meromorphic genus two Siegel modular forms of weight $2g-2$. They arise as Maass lifts of weak Jacobi forms of weight $2g-2$ and index 1 arising in an expansion of the elliptic genus in the equivariant parameter. We show the equivariant elliptic genus of $\mathbb{C}^{2}$ encodes the Gopakumar-Vafa invariants of $X_{\text{ban}}$. Therefore, one can regard $X_{\text{ban}}$ as an example where the generating functions of Gromov-Witten and Donaldson-Thomas invariants in fiber classes are produced by standard lifts of a modular object encoding the Gopakumar-Vafa invariants. We note that because this is a Masters thesis, the first six chapters offer an extended introduction to the relevant background material, while the original results are presented in the final chapter.

==> configuration.tex <==

\begin{figure}%\label{fig: banana configuration}
\centering
\begin{tikzpicture}[xshift=5cm,
                    %x  = {(-0.5cm,-0.5cm)},
                    %x  = {(-0.4,-1.0)},
                     %x  = {(1,-.25)},
                    %y  = {(2cm,0cm)},
                    %y  = {(0.5,1)},
                    %y  = {(0,1)},
                    %z  = {(0cm,1cm)},
                    %z  = {(1,1)},
                    %z  = {(-1,-1)},
                    %z  = {-15},
		    scale = 1.0
		    ]
%                    scale = 0.75]


\begin{scope}  
\draw (0,0) ellipse (2.4 and 2);
\draw (0,0) ellipse (0.6cm and 2cm);
\draw (0,0) ellipse (1.2cm and 2cm);
\draw (-0.6,0) arc(180:360:0.6 and 0.3);
\draw[dashed](-0.6,0) arc(180:0:0.6cm and 0.3cm);
\draw (1.2,0) arc(180:360:0.6cm and 0.3cm);
\draw[dashed](1.2,0) arc(180:0:0.6cm and 0.3cm);
\draw (-2.4,0) arc(180:360:0.6cm and 0.3cm);
\draw[dashed](-2.4,0) arc(180:0:0.6cm and 0.3cm);

\draw (0,-2) node[below] {$p$};
\draw(0,2) node[above] {$q$};
\draw(0,0.6) node {$C_{2}$};
\draw(-1.8,0.6) node {$C_{1}$};
\draw(1.8,0.6)node {$C_{3}$};
\end{scope}

%\draw[xshift=3.5cm,yshift=-2cm] (0,0)--(0,2)--(2,4)--(4,4)--(4,2)--(2,0)--(0,0);

\begin{scope}[xshift=4.5cm,yshift=-2cm]
\draw (0,1.5)--(1.5,1.5)--(2.5,2.5)--(4,2.5);
\draw (1.5,0)--(1.5,1.5)--(2.5,2.5)--(2.5,4);
\draw (0.5,1.5)node{$||$};
\draw (3.5,2.5)node{$||$};
\draw (1.5,0.5)node{$-$};
\draw (2.5,3.5)node{$-$};
\draw (2.5,3.1)node[left]{$C_{3}$};
\draw (2,2)node[below right]{$C_{2}$};
\draw (0.9,1.5)node[above]{$C_{1}$};
\draw (1.5,1.5)node[below left]{$p$};
\draw (2.5,2.5)node[above right]{$q$};
%\draw (-0.5,1)--(1,1)--(3,3)--(4.5,3);
%\draw (1,-0.5)--(1,1)--(3,3)--(3,4.5);
\end{scope}

\end{tikzpicture}
\caption{The banana configuration of $\PP^{1}$'s.  
}
\label{fig: banana configuration}
\end{figure}


